Design and control of a collision-resilient aerial vehicle with an icosahedron tensegrity structure

We introduce collision-resilient aerial vehicles with icosahedron tensegrity structures, capable of surviving high-speed impacts and resuming operations post-collision. We present a model-based design approach, which guides the selection of the tensegrity components by predicting structural stresses through a dynamics simulation. Furthermore, we develop an autonomous re-orientation controller that facilitates post-collision flight resumption. The controller enables the vehicles to rotate from an arbitrary orientation on the ground for takeoff. With collision resilience and re-orientation ability, the tensegrity aerial vehicles can operate in cluttered environments without complex collision-avoidance strategies. These capabilities are validated by a test of an experimental vehicle operating autonomously in a previously-unknown forest environment.

==> sections/deprecated/Sec2-TensegrityDesign_deprecated.tex <==
\label{sec:tensegrityDesign}
% Tensegrity vehicle design
% Includes:
% \begin{enumerate}
%     \item Basic idea, six-bar tensegrity + quad.
%     \item Collisions cause compression/tension stress Approx. stress analysis in a collision, corresponding design rules
%     \item Scaling analysis
% \end{enumerate}

In this section, we motivate the tensegrity aerial vehicle design, introduce the simplified stress analysis used to design the tensegrity, and analyze the relationship between scale and collision resilience of the design. The objective of the tensegrity shell is to protect the aerial vehicle against collisions. To achieve this, the tensegrity should not break during collisions and the deformation of the shell should be small so the external obstacles do not contact any parts originally inside the tensegrity shell.

We choose to design the collision-resilient aerial vehicle as a quadcopter, because its ability to hover and to vertically take off and land makes operation easier in cluttered environments. Differential flatness of the quadcopter also allows us to quickly plan trajectories and check their feasibility \cite{mueller2015computationally}. Meanwhile, we choose to protect the quadcopter with a 6-rod orthogonal icosahedron \cite{jessen1967orthogonal} tensegrity, because its shape is close to a sphere and can provide protection against collisions from all directions with the least amount of rods. % The center of mass of the icosahedron tensegrity also coincides with its geometric center and this makes hovering easier. 

We consider three factors when choosing components (rods and strings) to build the tension network of the tensegrity: weight, energy absorption ability, and stiffness. We prefer light components as they add less burden to flight and we wish components to absorb large energy during collision to make the vehicle collision-resilient. As for stiffness, we want stiff components with little flexibility for two advantages they bring. First, deformation of a stiff shell during collisions is small, so that the shell needs little buffer space to prevent propellers and electronics from being exposed. Hence, the tensegrity can be smaller in size and this helps the vehicle to fit through narrow gaps. Second, comparing to a tensegrity with components like springs, a stiff tensegrity experiences less internal vibration in the system, which leads to less disturbance during flight. The stiff shell design also brings a side bonus, that we can model the vehicle as a single rigid body. 



% \subsection{Quadcopter in icosahedron tensegrity}
% \subsection{Components of tension network}
% the magnitude of deformation during collisions, which is related to the stiffness of the component, and the agility of the vehicle, which is influenced by the weight of the component. We choose to build the tension network with stiff material because of two important advantages it brings. First, during a collision, deformation of a stiff shell is small and the shell needs little buffer space to prevent propellers and electronics from being exposed. As a result, the tensegrity size can be smaller in size and this helps the vehicle to fit through narrow gaps. Second, a stiff tensegrity experiences less low-frequency internal vibration in the system and thus adds less disturbance to the flight.

% Stiffness of the tensegrity shell reflects the trade-off between tensegrity's deformation and collision-resilience. A stiff tensegrity can absorb less energy than an elastic shell, but it also deforms less during collisions. Comparing to a tensegrity aerial vehicle with elastic components like springs, a stiff tensegrity aerial vehicle has two important advantages. First, during a collision, deformation of a stiff shell is small and the shell needs little buffer space to prevent propellers and electronics from being exposed. As a result, the tensegrity size can be smaller in size and this helps the vehicle to fit through narrow gaps. Second, a stiff tensegrity experiences less low-frequency internal vibration in the system and hence is expected to operate with more stability. We choose to design a vehicle with a stiff tensegrity shell because we are willing to sacrifice a part of energy-absorption capability for a smaller size and a better flight performance.

% The optimal stiffness of the tensegrity is 
% An elastic design is preferred for applications designed against extreme shocks,
% For applications designed against extreme shocks, like planetary landers \cite{rimoli2016impact} and aerial vehicles that may drop from high places \cite{fedorenko_2020}, elastic shells are preferred, because springs that can survive large shocks are much lighter than their stiff counterparts like metal cables. For a collision-resilient quadcopter, we design against lateral collisions which requires less shock absorption ability and springs no longer have weight advantage over stiff materials that can withstand the expected shock, such as braided wires and Kevlar cables. 

% Moreover, a stiff tensegrity aerial vehicle has two additional advantages. First, a stiff tensegrity can be smaller in size. Under the same external load, a stiff shell deforms less and hence needs less buffer room to prevent propellers and electronics from exposure. This allows the tensegrity design to be smaller and makes it easier to fit through narrow gaps. Second, a stiff tensegrity has less low frequency internal vibration in the system and hence will have less influence on flight performance of the aerial vehicle. Due to above advantages, we choose to design a vehicle with a stiff tensegrity shell.

\subsection{Simplified stress analysis}
% For a tensegrity to survive a collision, all of its components (rods and strings) need to survive the maximum compression and tension during the collision. We use a simplified stress analysis to approximate such load and predict if candidate tensegrity components can survive collisions of a given speed. 
% The analysis focuses on the moment when the tensegrity is under peak external impact. This impact can be approximated via dividing an conjectured change of linear momentum over collision time, or measured from drop tests of previous tensegrity prototypes of similar size and weight.

% As the distribution of the load within the tensegrity network depends on the stiffness of the components, the design process will be an iterative one. For each iteration, a candidate pair of rod and string is proposed, and then the maximum compression and tension in the network is computed. Afterwards, we determine if the proposed components can survive the collision by checking a list of criteria to be discussed in Section \ref{TensegrityComponentsCriteria}. 
% Methods of studying tensegrity systems during impact through dynamic simulation and finite element analysis have been proposed in \cite{rimoli2016impact} and \cite{pajunen2019design}.  

We introduce here a simplified stress analysis method to calculate the load in tensegrity components during collisions. We then use this analysis to predict if a candidate tensegrity component can survive collisions with a given speed. Two rules guide the selection of tensegrity components. First, the yielding strength and the buckling strength of each component should be larger than the maximum stress in the component. Second, the deformation of each component is smaller than a given maximum threshold so the parts originally inside the tensegrity shell will not be exposed. To further simplify the analysis, we make two additional assumptions. First, the weight of the tensegrity is much smaller than the impact force and thus can be ignored. Second, as the deformation of components is capped, we assume the shell can still maintain its orthogonal icosahedron geometry and we know the direction of all tension and compression forces in the structure. 

We define a tensegrity \emph{node} as a joint connecting a rod to strings. An icosahedron tensegrity has 12 nodes. For the stress analysis, we consider the following setup. Shown in Fig. \ref{StressAnalysis}, an icosahedron tensegrity is under external impact force with a sum of $F$. For our analysis, we evaluate $F$ as the average force of the collision. We study following scenarios: (a) only one node of the tensegrity is hitting the obstacle and the reaction force goes through the vehicle's center of mass, (b) two nodes of the tensegrity are hitting the obstacle and the reaction forces are parallel with the rods connected to the nodes, (c) a face with three nodes linked by two strings is hitting the obstacle, and (d) a face with three nodes linked by three strings is hitting the obstacle. We assume the load is evenly distributed among the contact nodes. We choose to analyze these collision configurations, because for other collision scenarios, the tensegrity will experience an external torque and the vehicle will rotate until the collision scenarios evolve into one of the configurations above.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{"figures/StressAnalysisSetup".pdf}
    \caption{Setup of the simplified stress analysis problem. We focus on the moment when the tensegrity shell undergoes the maximum impact load. Four configurations are considered: (a) The reaction force whose direction goes through center of mass acts on one of the tensegrity nodes. (b) Two reaction forces act on a pair of parallel rods. (c) Forces act on a face with two strings. (d) Forces act on a face with three strings.}
    \label{StressAnalysis}
\end{figure}

Denote the tensegrity nodes as $\boldsymbol{n}_i$, where $i = 1,...,12$. These nodes are connected by 6 rods and 20 strings. We denote the connectivity of the nodes with functions $N_r$ and $N_s$:
\begin{flalign}
 \label{connectivity_rod}
 & N_r(i,j)=   \begin{cases}
                                  1 \mbox{, if a rod connects
                                  $\boldsymbol{n}_i$ and $\boldsymbol{n}_j$} \\
                                  0 \mbox{, otherwise} 
  \end{cases} 
  \\
 \label{connectivity_string}
 & N_s(i,j)=   \begin{cases}
                                  1 \mbox{, if a string $l$ connects $\boldsymbol{n}_i$ and $\boldsymbol{n}_j$} \\
                                  0 \mbox{, otherwise} \\
  \end{cases}
\end{flalign}

Denote $T_{i,j}$ and $C_{i,j}$ respectively as the magnitude of the tensile force in string and compression force in rod connecting node $\boldsymbol{n}_i$ and $\boldsymbol{n}_j$. Use $\boldsymbol{u}_{i} \in \mathbb{R}^{3}$ to represent the external force on $\boldsymbol{n}_i$. Define  $\boldsymbol{e}_{i,j}$ as the unit vector from $\boldsymbol{n}_i$ to $\boldsymbol{n}_j$.

At the moment of the peak external load, we use a method similar to the one proposed in \cite{goyal2018dynamics} and derive equations of motion of the tensegrity system with Newton's second law. For each node $i$ we have:
\begin{align}
\sum_{j}-C_{i,j}N_r(i,j)\boldsymbol{e}_{i,j}+\sum_{j}-T_{i,j}N_s(i,j)\boldsymbol{e}_{i,j}+\boldsymbol{u}_{i} = m_i\cdot\boldsymbol{a}
% j|$\boldsymbol{N}_i^E $ \mbox{is connected to} $\boldsymbol{N}_i^E $ \} }
\label{ForceEq}
\end{align} 
where $m_i$ is the mass of the node $i$. To simplify the model, we assume that the mass of all parts of the vehicle are lumped to the 12 nodes of the tensegrity. Each node mass is computed as the sum of mass of all fasteners at the position of the node, half of the strings connected to the node, half of the rod connected to the node and all other parts (like motors, batteries, etc) mounted on that half of the rod. $\boldsymbol{a}$ is the acceleration of the tensegrity under external impact load. Its direction is assumed normal to the impact surface and and its magnitude can be calculated as:
\begin{align}
||\boldsymbol{a}|| = \frac{F}{\sum_i{m_i}}
\label{eq:accDuringCollision}
\end{align}

Due to the existence of self-stress (also known as pre-tension) in the icosahedron tensegrity, the structure is statically indeterminate. A detailed study of static indeterminacy of tensegrity structures can be found in \cite{pellegrino1986matrix}. With the assumption that the members of the tensegrity structure follow Hooke's law when the deformation is small, we solve for a minimum energy configuration solution with a method similar to the one proposed in \cite{monforton1980analysis}:
% the tensegrity structure is under minimum pre-stress, and that
\begin{align}
\begin{aligned}
\min_{T,C,\boldsymbol{u}} & \sum_{i,j} \frac{1}{2}  \Big(K_{r}(\epsilon_{i,j}L_r)^2N_r(i,j)  +  K_{s}(\epsilon_{i,j}L_s)^2N_s(i,j) \Big) \\
\textrm{s.t.  } & \text{Equations of motion: Eq. \eqref{ForceEq} }
\\
& \epsilon_{i,j} = \begin{cases}
                                  C_{i,j}/(E_rA_r) \mbox{, if $N_r(i,j) = 1$}\\
                                  T_{i,j}/(E_sA_s) \mbox{, if $N_s(i,j) = 1$}\\
                                  0 \mbox{, otherwise}
\end{cases}\\
& \epsilon_{i,j} \geq 0 \mbox{, if $N_s(i,j) = 1$}
\label{eq:optimizationStressAnalysis}
\end{aligned}
\end{align}
Constants $K$, $E$, $A$, $L$ denote Hooke's constant, Young's modulus, cross sectional area and length  respectively. Subscripts $s$ and $r$ represent string and rod respectively. $\epsilon_{i,j}$ is the strain of the component connecting node $i$ and node $j$. Notice that the strain of the string is constrained to be positive. This constrained optimization problem solves tension and compression corresponding to the minimum self-stress required so that no string turns slack during the collision. 

Comparing the results of all possible configurations, we find the maximum compression force in rods, $C_{max}$ and maximum tensile force in string-pieces, $T_{max}$. They are the maximum tensile and compression loads we expect the tensegrity to experience. We can predict if the candidate tensegrity components can survive these loads by checking the criteria below.

First, the stress in the string has to be smaller than its yielding strength $\sigma_{ys}$, with a factor of safety $\eta$: 
\begin{align}
\eta \frac{T_{max}}{A_s}  < \sigma_{ys}
\label{StringTensionLimit}
\end{align}
Meanwhile, the maximum stress in the rod should be smaller than both its yielding strength $\sigma_{yr}$ and its critical buckling strength $\sigma_{br}$ with a factor of safety:
\begin{align}
\eta \frac{C_{max}}{A_r}  < \textrm{min}(\sigma_{yr},\sigma_{br})
\label{RodCompressionLimit}
\end{align}
The yielding strength is a property of material, whereas the critical buckling strength of the rod can be found with Euler's buckling theory \cite{boresi1985advanced}: 
\begin{align}
\sigma_{br} = \frac{\pi^2E_rI_r}{A_r(L_r)^2}
\label{BucklingTheory}
\end{align}
here $I_r$ is the second moment of area of the rod. 
Last, the maximum deformation of the components needs to be under a small threshold length $L_t$ so that components inside the tensegrity will not contact obstacles during collision: 
\begin{align}
\frac{T_{max}}{E_sA_s}L_s < L_t,
\quad
\frac{C_{max}}{E_rA_r}L_r < L_t
\label{maxDeformation}
\end{align}

Thus Eq. \eqref{StringTensionLimit} to Eq. \eqref{maxDeformation} give us the bound that we need to design our vehicles around. This simplified stress analysis method gives us an easy-to-obtain guide to choose the components without relying on complicated FEA analysis. 


\subsection{Scaling analysis}
Tensegrity aerial vehicles of different sizes are needed to carry various payloads. In this subsection, we study the relationship between the scale of a tensegrity aerial vehicle and its collision resilience. In addition, we compare this relationship with that of a planar propeller guard, one of the most common protective structures for aerial vehicles. In this analysis, we define the size of a tensegrity aerial vehicle by its linear size scaling factor, $\lambda$ and hold constant the maximum thrust to weight ratio of the vehicle, which indicates the vehicle's agility. We then establish a relationship between the scaling factor and the vehicle's collision resilience, indicated by the maximum collision force the vehicle can survive.

Mach scaling \cite{wolowicz1979similitude} provides a relationship between maximum total thrust of the aerial vehicle and scaling factor. Mach scaling is used for compressible flow and suggests that the tip velocity of propellers is constant, and hence leads to $\omega \propto \frac{1}{\lambda}$, where $\omega$ is the angular velocity of the propeller. As propeller thrust is proportional to the square of the angular velocity of the propeller \cite{pounds2002design}, we have for the maximum thrust: 
\begin{align}
F_{max} \propto \omega_{max}^2\lambda^4 \propto \lambda^2
\label{maxThrustVSSize}
\end{align} 
As we assume the ratio between maximum total thrust and vehicle mass remains unchanged, the vehicle mass is a quadratic function of scaling factor:
\begin{align}
m = \kappa_1 \lambda^2
\label{totalMassVSSize}
\end{align} 
Assume the overall density of the quadcopter within the protective structure stays constant. So, the mass of the quadcopter grows cubically with the scale:
\begin{align}
m_q = \kappa_2 \lambda^3
\label{quadMassVSSize}
\end{align} 
Thus, the mass budget for the tensegrity shell, $m_t$ or the planar propeller guard, $m_g$ follows:
\begin{align}
% m_g = m_t = m - m_q = \kappa_1 \lambda^2 - \kappa_2 \lambda^3
m = \kappa_1 \lambda^2 - \kappa_2 \lambda^3
\label{tensegrityMassVSSize}
\end{align} 
This relationship suggests that the scale of the vehicle cannot grow infinitely. At the critical scale $\lambda = \kappa_1 / \kappa_2$, the mass budget for the protective structure goes to zero. 
% Now we consider the collision resilience of the scaled tensegrity structure. We use the impact model proposed in \cite{goldsmith1960impact} to estimate the relationship between peak force during impact and the impact object mass and impact velocity:
% \begin{align}
% F_p \propto  (m^3 v^6)^{\frac{1}{5}}
% \label{ElasticImpactTheory}
% \end{align} 
% where $F_p$ is the peak impact force and $v$ is the impact speed. 

Given the mass budget, we can find the maximum collision force the tensegrity shell can withstand. Let $F_{p}$ be the peak external force during collisions and let $C_{max}$ and $T_{max}$ be the maximum compression and tensile forces in the tensegrity system as the structure experiences the peak external force. The dynamics of the tensegrity system follows our previous analysis in Eq. \eqref{ForceEq}. Notice that the right hand side and the external force term $\boldsymbol{u}_i$ grows linearly with $F_{p}$. Thus, max tensile and compression force will also grow linearly with $F_{p}$:  
\begin{align}
C_{max}, T_{max} \propto F_{p}
\end{align} 
We assume the mass of strings are negligible comparing to that of rods in the tensegrity system. Therefore, the mass budget caps the collision resilience via capping the maximum force the rods can withstand. We assume the tensegrity rods are made with annular tubes, whose cross-sectional area and second moment of area are:  
\begin{align}
A_r = \pi(r_o^2-r_i^2), \quad
I_r = \frac{\pi}{2}(r_o^4-r_i^4) 
\label{AandI}
\end{align} 
where $r_o$ is the outer radius and $r_i$ is the inner radius. Assume both radius increase uniformly, i.e. $r_o \propto r_i$. Thus, we have $A_r \propto r_o^2$ and $I_r \propto r_o^4$. To survive the collision, the maximum stress in the rod should be smaller than its yielding strength and its critical buckling strength, as is described by Eq. \eqref{RodCompressionLimit}, \eqref{BucklingTheory}. As the tensegrity rods are slender, we assume the critical buckling strength is the limiting factor. We combine Eq. \eqref{RodCompressionLimit}, \eqref{BucklingTheory} with the scaling relationship of the rod's cross sectional area and the second moment of area, and get:
\begin{align}
I_r &\propto C_{max}L_r^2\\
\Rightarrow r_o^4 &\propto F_{p}L_r^2 \propto F_{p}\lambda^2 \\
\Rightarrow r_o &\propto (F_{p}\lambda^2)^{\frac{1}{4}}
\label{ro vs L}
\end{align} 
The relationship between the vehicle size and the tensegrity mass can hence be derived as:
\begin{align}
m_t \propto V_t \propto A_rL_r \propto r_o^2\lambda \propto (F_{p})^{\frac{1}{2}}\lambda^2
\label{mtVSSize1}
\end{align} 
Replacing the tensegrity mass term with Eq. \eqref{tensegrityMassVSSize}, we can thus get the relationship between vehicle scale and collision resilience for a tensegrity aerial vehicle under the assumption of constant maximum thrust to weight ratio: 
\begin{align}
F_p \propto (\kappa_1-\kappa_2\lambda)^2
\label{ForceVSScaleTensegrity}
\end{align} 

We investigate next the scaling relationship of planar propeller guards as a comparison. Propeller guards are most susceptible to bending moment during collisions and we will estimate its limit to find corresponding collision force. As the vehicle scales up, the length of the guard grows linearly so it can still enclose the propellers, i.e. $L_g \propto \lambda$. Assume the density of the propeller guard stays same. Since the structure is planar, we can relate the cross sectional area $A_g$ of the propeller guard with its total mass:
\begin{align}
A_g \propto \frac{V_g}{L_g} \propto \frac{m_g}{\lambda}   
\end{align}
We assume the maximum shear stress the propeller guard can withstand remains constant. So, the maximum shear force grows linearly with the guard's cross sectional area. We further assume the peak bending moment the structure can survive, $M_p$, is proportional to the maximum shear force. Furthermore, notice that the peak bending moment is a cross product of the moment arm, which scales linearly as $\lambda$, and the peak collision force. Thus we can find the scaling relationship for the peak collision force a planar propeller guard can withstand as: 

\begin{align}
F_p \propto \frac{M_{p}}{\lambda} \propto \frac{A_{g}}{\lambda} \propto \frac{m_g}{\lambda^2} \propto \kappa_1 - \kappa_2 \lambda
\label{scalingPropguard}
\end{align}  

Comparing relationship \eqref{ForceVSScaleTensegrity}, which is of a second order and \eqref{scalingPropguard}, which is affine, we can get a useful intuition for choosing protective structures during the design processes. Assume there exists a certain scale where both the tensegrity shell and the planar propeller guard can provide a same amount of collision resilience. Then, we want to protect the vehicle with a tensegrity shell if we wish to design a aerial vehicle of a smaller scale, because for a certain amount of decrease in the vehicle scale, the tensegrity shell will provide more increase in collision resilience.

==> sections/deprecated/Sec2-TensegrityDesign_deprecated2.tex <==
\label{sec:tensegrityDesign}
% Tensegrity vehicle design
% Includes:
% \begin{enumerate}
%     \item Basic idea, six-bar tensegrity + quad.
%     \item Collisions cause compression/tension stress Approx. stress analysis in a collision, corresponding design rules
%     \item Scaling analysis
% \end{enumerate}

In this section, we motivate the tensegrity aerial vehicle design, introduce the simplified stress analysis used to design the tensegrity, and analyze the relationship between scale and collision resilience of the design. The objective of the tensegrity shell is to protect the aerial vehicle against collisions. To achieve this, the tensegrity should not break during collisions and the deformation of the shell should be small so that the external obstacles do not contact any parts originally inside the tensegrity shell.

We choose to design the collision-resilient aerial vehicle as a quadcopter, because its ability to hover and to vertically take off and land makes operation easier in cluttered environments. Differential flatness of the quadcopter also allows us to quickly plan trajectories and check their feasibility \cite{mueller2015computationally}. Meanwhile, we choose to protect the quadcopter with a 6-rod orthogonal icosahedron \cite{jessen1967orthogonal} tensegrity, because its shape is close to a sphere and can provide protection against collisions from all directions with the least amount of rods. 

We consider three factors when choosing components (rods and strings) to build the tension network of the tensegrity: weight, energy absorption ability, and stiffness. We prefer light components as they add less burden to flight and we wish components to absorb large energy during collision to make the vehicle collision-resilient. As for stiffness, we prefer stiff components with little flexibility for two advantages they bring. First, deformation of a stiff shell during collisions is small, so the shell needs little buffer space to prevent propellers and electronics from being exposed. Hence, the tensegrity can be smaller in size and this helps the vehicle to fit through narrow gaps. Second, comparing to a tensegrity with components like springs, a stiff tensegrity experiences less internal vibration in the system, which leads to less disturbance during flights. 

% The stiff shell design also brings an additional bonus, that we can model the vehicle as a single rigid body. 



% \subsection{Quadcopter in icosahedron tensegrity}
% \subsection{Components of tension network}
% the magnitude of deformation during collisions, which is related to the stiffness of the component, and the agility of the vehicle, which is influenced by the weight of the component. We choose to build the tension network with stiff material because of two important advantages it brings. First, during a collision, deformation of a stiff shell is small and the shell needs little buffer space to prevent propellers and electronics from being exposed. As a result, the tensegrity size can be smaller in size and this helps the vehicle to fit through narrow gaps. Second, a stiff tensegrity experiences less low-frequency internal vibration in the system and thus adds less disturbance to the flight.

% Stiffness of the tensegrity shell reflects the trade-off between tensegrity's deformation and collision-resilience. A stiff tensegrity can absorb less energy than an elastic shell, but it also deforms less during collisions. Comparing to a tensegrity aerial vehicle with elastic components like springs, a stiff tensegrity aerial vehicle has two important advantages. First, during a collision, deformation of a stiff shell is small and the shell needs little buffer space to prevent propellers and electronics from being exposed. As a result, the tensegrity size can be smaller in size and this helps the vehicle to fit through narrow gaps. Second, a stiff tensegrity experiences less low-frequency internal vibration in the system and hence is expected to operate with more stability. We choose to design a vehicle with a stiff tensegrity shell because we are willing to sacrifice a part of energy-absorption capability for a smaller size and a better flight performance.

% The optimal stiffness of the tensegrity is 
% An elastic design is preferred for applications designed against extreme shocks,
% For applications designed against extreme shocks, like planetary landers \cite{rimoli2016impact} and aerial vehicles that may drop from high places \cite{fedorenko_2020}, elastic shells are preferred, because springs that can survive large shocks are much lighter than their stiff counterparts like metal cables. For a collision-resilient quadcopter, we design against lateral collisions which requires less shock absorption ability and springs no longer have weight advantage over stiff materials that can withstand the expected shock, such as braided wires and Kevlar cables. 

% Moreover, a stiff tensegrity aerial vehicle has two additional advantages. First, a stiff tensegrity can be smaller in size. Under the same external load, a stiff shell deforms less and hence needs less buffer room to prevent propellers and electronics from exposure. This allows the tensegrity design to be smaller and makes it easier to fit through narrow gaps. Second, a stiff tensegrity has less low frequency internal vibration in the system and hence will have less influence on flight performance of the aerial vehicle. Due to above advantages, we choose to design a vehicle with a stiff tensegrity shell.

\subsection{Simplified stress analysis}
% For a tensegrity to survive a collision, all of its components (rods and strings) need to survive the maximum compression and tension during the collision. We use a simplified stress analysis to approximate such load and predict if candidate tensegrity components can survive collisions of a given speed. 
% The analysis focuses on the moment when the tensegrity is under peak external impact. This impact can be approximated via dividing an conjectured change of linear momentum over collision time, or measured from drop tests of previous tensegrity prototypes of similar size and weight.

% As the distribution of the load within the tensegrity network depends on the stiffness of the components, the design process will be an iterative one. For each iteration, a candidate pair of rod and string is proposed, and then the maximum compression and tension in the network is computed. Afterwards, we determine if the proposed components can survive the collision by checking a list of criteria to be discussed in Section \ref{TensegrityComponentsCriteria}. 
% Methods of studying tensegrity systems during impact through dynamic simulation and finite element analysis have been proposed in \cite{rimoli2016impact} and \cite{pajunen2019design}.  

When a tensegrity is under external loads, it deforms itself in a way that minimizes the total energy stored in the system. According to the study on the stiffness of tensegrity structure in \cite{guest2011stiffness}, the deformation of the tensegrity comes from two parts: the change in length of tensegrity members (rods and strings), and the rotation of these members. We introduce here a simplified analysis method that solves an energy minimization problem with the orientation and the post-deformation length of tensegrity members as decision variables. From the solution, we can then extract the load in each tensegrity component and use it to predict if a candidate tensegrity component can survive collisions with a given speed. Two rules guide the selection process. First, the yielding strength and the buckling strength of each component should be larger than the maximum stress in the component. Second, the deformation of each component is smaller than a given threshold so the parts originally inside the tensegrity shell will not be exposed. To further simplify the analysis, we make two additional assumptions. First, the weight of the vehicle is much smaller than the impact force and can be ignored. Second, the members of the tensegrity follow the Hooke's law, so that the stress of each member is proportional to its strain.  

We define a tensegrity \emph{node} as a joint connecting a rod to strings. An icosahedron tensegrity has 12 nodes. For the stress analysis, we consider the following setup. Shown in Fig. \ref{StressAnalysis}, an icosahedron tensegrity is under external impact force with a sum of $F$. For our analysis, we evaluate $F$ as the average force of the collision. We study following scenarios: (a) only one node of the tensegrity is hitting the obstacle and the reaction force goes through the vehicle's center of mass, (b) two nodes of the tensegrity are hitting the obstacle and the reaction forces are parallel with the rods connected to the nodes, (c) a face with three nodes linked by two strings is hitting the obstacle, and (d) a face with three nodes linked by three strings is hitting the obstacle. We assume the load is evenly distributed among the contact nodes. We choose to analyze these collision configurations, because for other collision scenarios, the tensegrity will experience an external torque and the vehicle will rotate until the collision scenarios evolve into one of the configurations above.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{"figures/StressAnalysisSetup".pdf}
    \caption{Setup of the simplified stress analysis problem. We focus on the moment when the tensegrity shell undergoes the maximum impact load. Four configurations are considered: (a) The reaction force whose direction goes through center of mass acts on one of the tensegrity nodes. (b) Two reaction forces act on a pair of parallel rods. (c) Forces act on a face with two strings. (d) Forces act on a face with three strings.}
    \label{StressAnalysis}
\end{figure}
Denote the tensegrity nodes as $\boldsymbol{n}_i$, where $i = 1,...,12$. These nodes are connected by 6 rods and 20 strings. We denote the connectivity of the nodes with functions $N_r$ and $N_s$:
\begin{flalign}
 \label{connectivity_rod}
 & N_r(i,j)=   \begin{cases}
                                  1 \mbox{, if a rod connects
                                  $\boldsymbol{n}_i$ and $\boldsymbol{n}_j$} \\
                                  0 \mbox{, otherwise} 
  \end{cases} 
  \\
 \label{connectivity_string}
 & N_s(i,j)=   \begin{cases}
                                  1 \mbox{, if a string $l$ connects $\boldsymbol{n}_i$ and $\boldsymbol{n}_j$} \\
                                  0 \mbox{, otherwise} \\
  \end{cases}
\end{flalign}

We define $T_{i,j}$ and $C_{i,j}$ respectively as the magnitude of the tensile force in string and compression force in rod connecting node $\boldsymbol{n}_i$ and $\boldsymbol{n}_j$. They can be calculated from the Hooke's law: 
\begin{align}
T_{i,j} = K_s \delta L_{i,j} = K_s(L_{i,j} - L_s)\label{tensile force}\\
C_{i,j} = K_r \delta L_{i,j} = K_r(L_r -L_{i,j})
\label{compression forece}
\end{align}
where $K_s$ and $K_r$ are the Hooke's coefficients of the string and the rod. $\delta L_{i,j}$ is the length deformation of the tensegrity member connecting node $\boldsymbol{n}_i$ and $\boldsymbol{n}_j$. It can be computed as the difference between $L_{i,j}$, the corresponding length under external load, and $L_s$ or $L_r$, the original string or rod length without any deformation. 

Let $\boldsymbol{u}_{i} \in \mathbb{R}^{3}$ represent the external collision force on $\boldsymbol{n}_i$. Define  $\boldsymbol{e}_{i,j}$ as the unit vector pointing from $\boldsymbol{n}_i$ to $\boldsymbol{n}_j$. When the tensegrity is under the external load due to collision, we use a method similar to the one proposed in \cite{goyal2018dynamics} and derive equations of motion of the tensegrity system with Newton's second law for each node $i$:
\begin{align}
\sum_{j}-C_{i,j}N_r(i,j)\boldsymbol{e}_{i,j}+\sum_{j}T_{i,j}N_s(i,j)\boldsymbol{e}_{i,j}+\boldsymbol{u}_{i} = m_i\cdot\boldsymbol{a}
\label{ForceEq}
\end{align} 
where $m_i$ is the mass of the node $i$. To simplify the analysis, we assume that the mass of the vehicle is lumped to the nodes of the tensegrity. Each node mass is approximated as the sum of mass of all fasteners at the position of the node, half of the strings connected to the node, half of the rod connected to the node and all other parts (motors, batteries, etc) mounted on that half of the rod. $\boldsymbol{a}$ is the acceleration of the tensegrity under external impact load. Its direction is assumed normal to the impact surface and and its magnitude can be calculated as:
\begin{align}
||\boldsymbol{a}|| = \frac{F}{\sum_i{m_i}}
\label{eq:accDuringCollision}
\end{align}
As we expect the tensegrity to be stiff and the overall behavior of the tensegrity to be like a rigid body, we assume here the acceleration of all nodes are equal.

In addition to the equations of motion, the tensegrity also follows the topology constraint that each triangle on the tensegrity surface will remain a triangle after deformation. Let $\boldsymbol{n}_i$, $\boldsymbol{n}_j$, and $\boldsymbol{n}_k$ be three nodes that are connected by three tensegrity members so that they form a triangle. They should still form a triangle after deformation: 
\begin{align}
L_{i,j}\boldsymbol{e}_{i,j} + L_{j,k}\boldsymbol{e}_{j,k} +
L_{k,i}\boldsymbol{e}_{k,i}= \boldsymbol{0}
\label{eq:topology constraint}
\end{align} 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{"figures/ToplogyConstraint".pdf}
    \caption{Examples for triangles on tensegrity surfaces. Left: a triangle made with three nodes connected by three strings. Right: a triangle made with three nodes connected by two strings and a rod.}
    \label{topology constraint}
\end{figure}
A visual example of tensegrity surface triangles can be found in Fig.\ref{topology constraint}. On an icosahedron tensegrity, there are 8 triangles formed with 3 strings and 12 triangles formed with 2 strings and 1 rod. So there are in total twenty topology constraint equations.  

Now, we can solve for a minimum energy tensegrity configuration after deformation, with the length and directions of tensegrity members as decision variables, and subject to the equations of motion and the topology constraints. 
\begin{align}
\begin{aligned}
\min_{L, \boldsymbol{e}} \frac{1}{2} \sum_{i,j}   & K_{r}(L_{i,j}-L_r)^2N_r(i,j) +  K_{s}(L_{i,j}-L_s)^2N_s(i,j)\\
\textrm{s.t.  } & \text{Equations of motion: Eq. \eqref{ForceEq} }\\
& \text{Topology constraint: Eq. \eqref{eq:topology constraint}}\\
& L_{i,j} - L_s \geq 0 \mbox{, if $N_s(i,j) = 1$}\\
& ||\boldsymbol{e}_{i,j}|| = 1 \mbox{, if $N_s(i,j) = 1$ or $N_r(i,j) = 1$}
\label{eq:optimizationStressAnalysis}
\end{aligned}
\end{align}
The last two constraints assert that the strings cannot be compressed and the direction vectors are unit vectors.


After solving the optimization problem, we can compute the tensile and compression forces with eq. \eqref{tensile force},\eqref{compression forece}.
Comparing the results of all possible collision configurations, we find the maximum compression force in rods, $C_{max}$ and maximum tensile force in string-pieces, $T_{max}$. They are the maximum tensile and compression loads we expect the tensegrity to experience. We can predict if the candidate tensegrity components can survive these loads by checking the criteria below. 

We use $A$, $E$, $I$ to denote the cross sectional area, Young's modulus and second moment of area. We also use subscript $r$ for characteristics related to rods and $s$ for ones related to strings. First, the stress in the string has to be smaller than its yielding strength $\sigma_{ys}$, with a factor of safety $\eta$: 
\begin{align}
\eta \frac{T_{max}}{A_s}  < \sigma_{ys}
\label{StringTensionLimit}
\end{align}
Meanwhile, the maximum stress in the rod should be smaller than both its yielding strength $\sigma_{yr}$ and its critical buckling strength $\sigma_{br}$ with a factor of safety:
\begin{align}
\eta \frac{C_{max}}{A_r}  < \textrm{min}(\sigma_{yr},\sigma_{br})
\label{RodCompressionLimit}
\end{align}
The yielding strength is a property of material, whereas the critical buckling strength of the rod can be found with Euler's buckling theory \cite{boresi1985advanced}: 
\begin{align}
\sigma_{br} = \frac{\pi^2E_rI_r}{A_r(L_r)^2}
\label{BucklingTheory}
\end{align}
Last, the maximum deformation of the components needs to be under a small threshold length $L_t$ so that components inside the tensegrity will not contact obstacles during collision: 
\begin{align}
\frac{T_{max}}{E_sA_s}L_s < L_t,
\quad
\frac{C_{max}}{E_rA_r}L_r < L_t
\label{maxDeformation}
\end{align}

Thus Eq. \eqref{StringTensionLimit} to Eq. \eqref{maxDeformation} give us the bound that we need to design our vehicles around. This simplified stress analysis method gives us a quick guide to choose the components without relying on complicated FEA analysis. 


% \subsection{Scaling analysis}
% Tensegrity aerial vehicles of different sizes are needed to carry various payloads. In this subsection, we study the relationship between the scale of a tensegrity aerial vehicle and its collision resilience. In addition, we compare this relationship with that of a planar propeller guard, one of the most common protective structures for aerial vehicles. In this analysis, we define the size of a tensegrity aerial vehicle by its linear size scaling factor, $\lambda$ and hold constant the maximum thrust to weight ratio of the vehicle, which indicates the vehicle's agility. We then establish a relationship between the scaling factor and the vehicle's collision resilience, indicated by the maximum collision force the vehicle can survive.

% Mach scaling \cite{wolowicz1979similitude} provides a relationship between maximum total thrust of the aerial vehicle and scaling factor. Mach scaling is used for compressible flow and suggests that the tip velocity of propellers is constant, and hence leads to $\omega \propto \frac{1}{\lambda}$, where $\omega$ is the angular velocity of the propeller. As propeller thrust is proportional to the square of the angular velocity of the propeller \cite{pounds2002design}, we have for the maximum thrust: 
% \begin{align}
% F_{max} \propto \omega_{max}^2\lambda^4 \propto \lambda^2
% \label{maxThrustVSSize}
% \end{align} 
% As we assume the ratio between maximum total thrust and vehicle mass remains unchanged, the vehicle mass is a quadratic function of scaling factor:
% \begin{align}
% m = \kappa_1 \lambda^2
% \label{totalMassVSSize}
% \end{align} 
% Assume the overall density of the quadcopter within the protective structure stays constant. So, the mass of the quadcopter grows cubically with the scale:
% \begin{align}
% m_q = \kappa_2 \lambda^3
% \label{quadMassVSSize}
% \end{align} 
% Thus, the mass budget for the tensegrity shell, $m_t$ or the planar propeller guard, $m_g$ follows:
% \begin{align}
% % m_g = m_t = m - m_q = \kappa_1 \lambda^2 - \kappa_2 \lambda^3
% m = \kappa_1 \lambda^2 - \kappa_2 \lambda^3
% \label{tensegrityMassVSSize}
% \end{align} 
% This relationship suggests that the scale of the vehicle cannot grow infinitely. At the critical scale $\lambda = \kappa_1 / \kappa_2$, the mass budget for the protective structure goes to zero. 
% % Now we consider the collision resilience of the scaled tensegrity structure. We use the impact model proposed in \cite{goldsmith1960impact} to estimate the relationship between peak force during impact and the impact object mass and impact velocity:
% % \begin{align}
% % F_p \propto  (m^3 v^6)^{\frac{1}{5}}
% % \label{ElasticImpactTheory}
% % \end{align} 
% % where $F_p$ is the peak impact force and $v$ is the impact speed. 

% Given the mass budget, we can find the maximum collision force the tensegrity shell can withstand. Let $F_{p}$ be the peak external force during collisions and let $C_{max}$ and $T_{max}$ be the maximum compression and tensile forces in the tensegrity system as the structure experiences the peak external force. The dynamics of the tensegrity system follows our previous analysis in Eq. \eqref{ForceEq}. Notice that the right hand side and the external force term $\boldsymbol{u}_i$ grows linearly with $F_{p}$. Thus, max tensile and compression force will also grow linearly with $F_{p}$:  
% \begin{align}
% C_{max}, T_{max} \propto F_{p}
% \end{align} 
% We assume the mass of strings are negligible comparing to that of rods in the tensegrity system. Therefore, the mass budget caps the collision resilience via capping the maximum force the rods can withstand. We assume the tensegrity rods are made with annular tubes, whose cross-sectional area and second moment of area are:  
% \begin{align}
% A_r = \pi(r_o^2-r_i^2), \quad
% I_r = \frac{\pi}{2}(r_o^4-r_i^4) 
% \label{AandI}
% \end{align} 
% where $r_o$ is the outer radius and $r_i$ is the inner radius. Assume both radius increase uniformly, i.e. $r_o \propto r_i$. Thus, we have $A_r \propto r_o^2$ and $I_r \propto r_o^4$. To survive the collision, the maximum stress in the rod should be smaller than its yielding strength and its critical buckling strength, as is described by Eq. \eqref{RodCompressionLimit}, \eqref{BucklingTheory}. As the tensegrity rods are slender, we assume the critical buckling strength is the limiting factor. We combine Eq. \eqref{RodCompressionLimit}, \eqref{BucklingTheory} with the scaling relationship of the rod's cross sectional area and the second moment of area, and get:
% \begin{align}
% I_r &\propto C_{max}L_r^2\\
% \Rightarrow r_o^4 &\propto F_{p}L_r^2 \propto F_{p}\lambda^2 \\
% \Rightarrow r_o &\propto (F_{p}\lambda^2)^{\frac{1}{4}}
% \label{ro vs L}
% \end{align} 
% The relationship between the vehicle size and the tensegrity mass can hence be derived as:
% \begin{align}
% m_t \propto V_t \propto A_rL_r \propto r_o^2\lambda \propto (F_{p})^{\frac{1}{2}}\lambda^2
% \label{mtVSSize1}
% \end{align} 
% Replacing the tensegrity mass term with Eq. \eqref{tensegrityMassVSSize}, we can thus get the relationship between vehicle scale and collision resilience for a tensegrity aerial vehicle under the assumption of constant maximum thrust to weight ratio: 
% \begin{align}
% F_p \propto (\kappa_1-\kappa_2\lambda)^2
% \label{ForceVSScaleTensegrity}
% \end{align} 

% We investigate next the scaling relationship of planar propeller guards as a comparison. Propeller guards are most susceptible to bending moment during collisions and we will estimate its limit to find corresponding collision force. As the vehicle scales up, the length of the guard grows linearly so it can still enclose the propellers, i.e. $L_g \propto \lambda$. Assume the density of the propeller guard stays same. Since the structure is planar, we can relate the cross sectional area $A_g$ of the propeller guard with its total mass:
% \begin{align}
% A_g \propto \frac{V_g}{L_g} \propto \frac{m_g}{\lambda}   
% \end{align}
% We assume the maximum shear stress the propeller guard can withstand remains constant. So, the maximum shear force grows linearly with the guard's cross sectional area. We further assume the peak bending moment the structure can survive, $M_p$, is proportional to the maximum shear force. Furthermore, notice that the peak bending moment is a cross product of the moment arm, which scales linearly as $\lambda$, and the peak collision force. Thus we can find the scaling relationship for the peak collision force a planar propeller guard can withstand as: 

% \begin{align}
% F_p \propto \frac{M_{p}}{\lambda} \propto \frac{A_{g}}{\lambda} \propto \frac{m_g}{\lambda^2} \propto \kappa_1 - \kappa_2 \lambda
% \label{scalingPropguard}
% \end{align}  

% Comparing relationship \eqref{ForceVSScaleTensegrity}, which is of a second order and \eqref{scalingPropguard}, which is affine, we can get a useful intuition for choosing protective structures during the design processes. Assume there exists a certain scale where both the tensegrity shell and the planar propeller guard can provide a same amount of collision resilience. Then, we want to protect the vehicle with a tensegrity shell if we wish to design a aerial vehicle of a smaller scale, because for a certain amount of decrease in the vehicle scale, the tensegrity shell will provide more increase in collision resilience.

==> sections/deprecated/oldScalingAnalysis.tex <==
\subsection{Scaling analysis}
Tensegrity aerial vehicles of different sizes are needed to carry various payloads. We are interested in the relationship between the scale of tensegrity aerial vehicles and their agility, and how this scaling relationship compares with that of a normal quadcopter and other protection structures. We define the size of the vehicle by its linear size scaling factor, $\lambda$, hold constant the maximum collision speed the vehicle can survive, and find a relationship between $\lambda$ and the ratio of tensegrity weight over maximum thrust. We then compare this scaling relationship with that of a quadcopter without a tensegrity shell and a quadcopter with a propeller guard. Our analysis shows that tensegrity structure is more favorable than common planar protection structure like propeller guards as the vehicle scales up.

We first apply Mach scaling \cite{wolowicz1979similitude} to approximate the relationship between maximum total thrust and scaling factor. Mach scaling is used for compressible flow and suggests that the tip velocity of propellers is constant, and hence leads to $\omega \propto \frac{1}{\lambda}$, where $\omega$ is the angular velocity of the propeller. As propeller thrust is proportional to the square of the angular velocity of the propeller \cite{pounds2002design}, we have for the maximum thrust, 
\begin{align}
F_{max} \propto \omega_{max}^2\lambda^4 \propto \lambda^2
\label{maxThrustVSSize}
\end{align} 

Assume the overall density of a normal quadcopter remains same as it scales up. So, the mass of a normal quadcopter grows cubically as the scale of the vehicle, i.e. $m_v \propto \lambda ^3$. Thus the relationship between a quadcopter's weight and its scale is:
\begin{align}
\frac{w_q}{F_{max}} = \frac{m_q||\boldsymbol{g}||}{F_{max}} \propto \frac{m_q}{\lambda^2} \propto \lambda
\label{scalingQuad}
\end{align} 
where $\boldsymbol{g}$ is the gravitational acceleration, $w_q$ and $m_q$ are the weight and mass of the quadcopter respectively.

Now we consider the tensegrity aerial vehicle. We use the impact model proposed in \cite{goldsmith1960impact} to estimate the relationship between peak force during impact and the impact object mass and impact velocity:
\begin{align}
F_p \propto  (m^3 v^6)^{\frac{1}{5}}
\label{ElasticImpactTheory}
\end{align} 
where $F_p$ is the peak impact force, $m$ is the mass of the object impact against a large obstacle and $v$ is the impact speed. We assume that the overall density of the vehicle will stay same and its mass will grow cubically with its size, i.e. $m\propto \lambda^3$. Moreover, as the impact speeds are held constant, we have:
\begin{align}
F_p \propto (\lambda)^{\frac{9}{5}}
\label{PeakForceVSSize}
\end{align} 

We then consider the maximum compression force, $C_{max}$ and tension, $T_{max}$ in the tensegrity system as the structure experiences maximum external load $F_{p}$ during a collision. The system follows Eq. \eqref{ForceEq}. The right hand side and the external force term $\boldsymbol{u}_i$ grows linearly with $F_{p}$, and the $\boldsymbol{r}_{i,j},\boldsymbol{s}_{i,j}$ terms remains constant. Thus, we expect max tensile and compression force to grow linearly with $F_{p}$:  
\begin{align}
C_{max}, T_{max} \propto F_{p}
\end{align} 

On the other hand, tensegrity rods are made with tube with an annular shape. Thus, we have:  
\begin{align}
A = \pi(r_o^2-r_i^2)\\
I = \frac{\pi}{2}(r_o^4-r_i^4) 
\label{AandI}
\end{align} 
where $r_o$ is the outer radius and $r_i$ is the inner radius. Assume outer and inner radius increases uniformly, i.e. $r_o \propto r_i$. Thus, we have $A \propto r_o^2$ and $I \propto r_o^4$. 

To survive the collision, the maximum stress in the rod should be smaller than its critical buckling strength, as is described by Eq. \eqref{RodCompressionLimit}, \eqref{BucklingTheory}.
% \begin{align}
% A = \pi(2r_oc+c^2)\\
% I = 4r_o^3c-4r_o^2c^2+4r_oc^3-c^4
% \label{RodCompressionLimit}
% \end{align} 
% As the tensegrity structures are made with carbon fiber tubes, which are rolled carbon fiber sheets with a small constant thickness. Hence, we have $r_i = r_o -c$, where $c$ is a small constant representing the thickness of carbon fiber sheet. Replace $r_i$ in previous equations:
% \begin{align}
% A = \pi(2r_oc+c^2)\\
% I = 4r_o^3c-4r_o^2c^2+4r_oc^3-c^4
% \label{RodCompressionLimit}
% \end{align} 
% As c is a small number, we approximate the cross sectional area and moment of area with the highest order of polynomial of the outer diameter. Hence, $A \tilde{\propto} r_o$ and $I \widetilde{\propto} r_o^3$.
We plug in the relationships about peak external load, rod cross sectional area and moment of inertia into these constraints, and get:
\begin{align}
I \propto C_{max}L^2\\
\Rightarrow r_o^4 \propto F_{p}L^2 \propto F_{p}\lambda^2 \\
\Rightarrow r_o \propto (F_{p}\lambda^2)^{\frac{1}{4}}
% \Rightarrow r_o \propto \lambda^\frac{7}{6} (\text{  if} F_{max} \propto \lambda^{\frac{3}{2}})
\label{ro vs L}
\end{align} 
The relationship between the vehicle size and the tensegrity mass can then be derived as:
\begin{align}
m_t \propto V_t \propto AL \propto r_o^2\lambda \propto (F_{p}\lambda^2)^{\frac{1}{2}}\lambda
% \text{with model:} F_{max} \propto \lambda^{\frac{3}{2} }\\
% \Rightarrow m_t \propto \lambda^{\frac{13}{6}}
\label{mtVSSize1}
\end{align} 

We plug in the relationship \eqref{PeakForceVSSize}, and get: 
\begin{align}
m_t \propto \lambda^{\frac{29}{10}}
\label{mtVSSize2}
\end{align} 

We plug in relationship \eqref{maxThrustVSSize}, and the ratio between the tensegrity shell's weight and the maximum thrust is:
\begin{align}
\frac{w_t}{F_{max}} = \frac{m_t||\boldsymbol{g}||}{F_{max}} \propto \frac{m_t}{\lambda^2} \propto \lambda^{\frac{9}{10}}
\label{scalingTensegrityShell}
\end{align}  

Last, we consider scaling of the most common non-tensegrity protection structure, planar propeller guard, as comparison. Unlike tensegrity, propeller guards are susceptible to bending moment during collisions. As the vehicle scales up, the length of the guard grows linearly so it can still enclose the propellers, i.e. $L_g \propto \lambda$. With peak force relationship \eqref{ElasticImpactTheory}, we can further obtain the relationship between peak bending moment and the scaling factor: 
\begin{align}
M_p \propto F_{p}L_n \propto 
\lambda^{\frac{9}{5}}\cdot \lambda = \lambda^{\frac{14}{5}}
\label{scalingM_propguard}
\end{align}  

We further assume the max shear force in the structure grows linearly as the peak bending moment. To survive this shear, the cross sectional area of the structure has to scale up:  
\begin{align}
A_g \propto V_{max} \propto M_p \propto \lambda^{\frac{14}{5}}
\label{scalingA_propguard}
\end{align}  
Hence, the weight to max total thrust ratio of a planar propeller guard scales as:
\begin{align}
\frac{w_g}{F_{max}} = \frac{m_g||\boldsymbol{g}||}{F_{max}} \propto \frac{A_gL_g}{F_{max}} \propto \frac{\lambda^{\frac{14}{5}}\cdot \lambda}{\lambda^2} \propto \lambda^{\frac{9}{5}}
\label{scalingNonTensegrityShell}
\end{align}  



Comparing the relationship \eqref{scalingNonTensegrityShell}, \eqref{scalingTensegrityShell} and \eqref{scalingQuad}, we find that as the vehicle scales up, the ratio between tensegrity shell's weight and max total thrust grows slower than that of both normal quadcopters and planar propeller guards. As a result, scaling up the tensegrity aerial vehicle will not lead to more agility loss than scaling up a normal quadcopter or a quadcopter with planar protections such as propeller guards.

% Notice that the scaling analysis here is specific to rigid tensegrity shells and it aims to provide an intuition, instead of a design guidance. Specific design decisions still needs to be made for vehicles of various sizes, as the dimension of available components usually do not grow continuously. Moreover, the design may meet additional non-mechanical constraints, such as the maximum current the battery can provide.


% What is the advantage of elastic shell? Can store energy via deformation. So can get away with lighter material. But you need to be larger in size. So whether a the total mass will decrease is up in the air. 

